Deformable One-shot Face Stylization via DINO Semantic Guidance

This paper addresses the complex issue of one-shot face stylization, focusing on the simultaneous consideration of appearance and structure, where previous methods have fallen short. We explore deformation-aware face stylization that diverges from traditional single-image style reference, opting for a real-style image pair instead. The cornerstone of our method is the utilization of a self-supervised vision transformer, specifically DINO-ViT, to establish a robust and consistent facial structure representation across both real and style domains. Our stylization process begins by adapting the StyleGAN generator to be deformation-aware through the integration of spatial transformers (STN). We then introduce two innovative constraints for generator fine-tuning under the guidance of DINO semantics: i) a directional deformation loss that regulates directional vectors in DINO space, and ii) a relative structural consistency constraint based on DINO token self-similarities, ensuring diverse generation. Additionally, style-mixing is employed to align the color generation with the reference, minimizing inconsistent correspondences. This framework delivers enhanced deformability for general one-shot face stylization, achieving notable efficiency with a fine-tuning duration of approximately 10 minutes. Extensive qualitative and quantitative comparisons demonstrate our superiority over state-of-the-art one-shot face stylization methods. Code is available at https://github.com/zichongc/DoesFS

==> tables/eval_id.tex <==

\begin{table}
\small
\caption{
\textbf{Quantitative evaluation of methods by directional ID similarity ($\uparrow$).} We choose three style examples as shown in Fig.\ref{fig:cmp_unpair} top for evaluation, and they are represented by Example1, Example2 and Example3 from left to right, respectively. Best results are \textbf{blod} and second-best are \underline{underlined}. 
}
\label{tab:id}
\vspace*{-5mm}
\begin{center}
\begin{tabular}{r|ccc}
  \Xhline{1pt}
  Method & Example1 & Example2 &Example3 \\ \Xhline{0.6pt}
  MTG \cite{zhu2022mtg} & 0.264 & 0.301 & 0.254   \\
  JoJoGAN \cite{chong2022jojogan} & 0.290 & 0.378 & \underline{0.382}  \\
  DiFa \cite{zhang2022towards} & 0.223 & 0.328 & 0.123   \\
  OneshotCLIP \cite{guhyun2023oneshotclip} & 0.333 & 0.113 & 0.201   \\ \Xhline{0.6pt}
  MTG-pair & 0.392 & 0.335 & 0.280  \\
  JoJoGAN-pair & \underline{0.405} & \textbf{0.393} & \textbf{0.400}  \\ \Xhline{0.6pt}
  Ours & \textbf{0.468} & \underline{0.379} & 0.330  \\
  \Xhline{1pt}
\end{tabular} 
\end{center}
\end{table}
%\vspace{-0.3cm}


==> tables/eval_lpips.tex <==

\begin{table*}%
\small
\caption{
\textbf{Quantitative evaluation of methods by LPIPS ($\downarrow$) and Cross-LPIPS error  ($\downarrow$).} We choose three style examples as shown in Fig.\ref{fig:cmp_unpair} top for evaluation, and they are represented by Example1, Example2 and Example3 from left to right, respectively. Best results are \textbf{blod} and second-best are \underline{underlined}. 
}
\label{tab:lpips}
% \begin{minipage}{\columnwidth}
\vspace*{-5mm}
\begin{center}
\begin{tabular}{r|ccc|ccc|ccc}

  \Xhline{1pt}
  \multirow{2}*{Method} & \multicolumn{3}{c|}{Example1} & \multicolumn{3}{c|}{Example2} & \multicolumn{3}{c}{Example3} \\ \cline{2-10}
  ~ & LPIPS $\downarrow$ & \makecell{Cross-LPIPS\\ err. $\downarrow$} & \makecell{dir-ID\\ sim. $\uparrow$} & LPIPS $\downarrow$ & \makecell{Cross-LPIPS\\ err. $\downarrow$} & \makecell{dir-ID\\ sim. $\uparrow$} & LPIPS $\downarrow$ & \makecell{Cross-LPIPS\\ err. $\downarrow$} & \makecell{dir-ID\\ sim. $\uparrow$} \\ \Xhline{0.6pt}
  MTG \cite{zhu2022mtg} & \textbf{0.340} & 0.055 & 0.264 & \underline{0.361} & 0.064 & 0.301 &\textbf{0.328} & 0.056 & 0.254 \\
  JoJoGAN \cite{chong2022jojogan} & 0.357 & 0.049 & 0.290 & 0.385 & 0.049 & 0.378 & 0.355 & \underline{0.044} & \underline{0.382} \\
  DiFa \cite{zhang2022towards} & 0.362 & 0.048 & 0.223 & \textbf{0.293} & 0.118 & 0.328 & 0.346 & 0.048 & 0.123 \\
  OneshotCLIP \cite{guhyun2023oneshotclip} & 0.452 & 0.080 & 0.333 & 0.449 & 0.059 & 0.113 & 0.460 & 0.097 & 0.201 \\ \cline{1-10}
  MTG-pair & 0.423 & 0.054 & 0.392 & 0.447 & 0.050 & 0.335 & 0.379 & 0.045 & 0.280 \\
  JoJoGAN-pair & 0.381 & \textbf{0.045} & \underline{0.405} & 0.395 & \textbf{0.041} & \textbf{0.393} & 0.383 & 0.045 
& \textbf{0.400} \\ \cline{1-10}
  Ours & \underline{0.353} & \underline{0.046} & \textbf{0.468} & 0.379 & \underline{0.048} & \underline{0.379} & \underline{0.342} & \textbf{0.041} & 0.330 \\
  
  \Xhline{1pt}
  % \hline
\end{tabular} 
\end{center}
% \end{minipage}
\end{table*}%
%\vspace{-0.3cm}

==> tables/eval_pair.tex <==

% % v1
% \begin{table*}[htbp]%
% \small 
% \caption{
% \textbf{Quantitative evaluation.} We choose the three styles shown in Fig.~\ref{fig:cmp_unpair} for evaluation, which are represented as Example-1, Example-2 and Example-3 from left to right, respectively. The best results are \textbf{blod}, and the second-bests are \underline{underlined}. 
% } % of methods by three metrics
% \label{tab:eval}
% % \begin{minipage}{\columnwidth}
% \vspace*{-5mm}
% \begin{center}
% \begin{tabular}{r|ccc|ccc|ccc}

%   \Xhline{1pt}
%   \multirow{2}*{Method} & \multicolumn{3}{c|}{Example-1} & \multicolumn{3}{c|}{Example-2} & \multicolumn{3}{c}{Example-3} \\ \cline{2-10}
%   ~ & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} \\ \Xhline{0.6pt}
%   % MTG \cite{zhu2022mtg} & \textbf{0.340} & 0.123 & 0.264 & \underline{0.361} & 0.111 & 0.301 &\textbf{0.328} & 0.095 & 0.254 \\
%   % JoJoGAN \cite{chong2022jojogan} & 0.357 & 0.149 & 0.290 & 0.385 & 0.138 & 0.378 & 0.355 & 0.097 & \underline{0.382} \\
%   % DiFa \cite{zhang2022towards} & 0.362 & 0.142 & 0.223 & \textbf{0.293} & 0.137 & 0.328 & 0.346 & 0.094 & 0.123 \\
%   % OneshotCLIP \cite{guhyun2023oneshotclip} & 0.452 & 0.157 & 0.333 & 0.449 & 0.119 & 0.113 & 0.460 & 0.136 & 0.201 \\ \cline{1-10}
%   MTG-pair & 0.423 & \underline{0.195} & 0.392 & 0.447 & \underline{0.174} & 0.335 & 0.379 & 0.159 & 0.280 \\
%   JoJoGAN-pair & 0.381 & 0.180 & \underline{0.405} & 0.395 & 0.155 & \textbf{0.393} & 0.383 & \underline{0.173} 
% & \textbf{0.400} \\ %\cline{1-10}
%   Ours & \underline{0.353} & \textbf{0.196} & \textbf{0.468} & 0.379 & \textbf{0.194} & \underline{0.379} & \underline{0.342} & \textbf{0.191} & 0.330 \\
  
%   \Xhline{1pt}
%   % \hline
% \end{tabular} 
% \end{center}
% % \end{minipage}
% \vspace*{-3mm}
% \end{table*}%
% %\vspace{-0.3cm}







% v2

\begin{table}[htbp]%
\small 
\caption{
\textbf{Quantitative comparison with ``paired'' variants} of MTG~\cite{zhu2022mtg} and JoJoGAN~\cite{chong2022jojogan} on the three styles shown in Fig.~\ref{fig:cmp_unpair}.
%We choose the three styles shown in Fig.~\ref{fig:cmp_unpair} for evaluation, which are represented as Example-1, Example-2 and Example-3 from left to right, respectively. The best results are \textbf{blod}, and the second-bests are \underline{underlined}. 
} % of methods by three metrics
\label{tab:eval_pair}
% \begin{minipage}{\columnwidth}
\vspace*{-5mm}
\begin{center}
\begin{tabular}{cc|ccc}
  \Xhline{1pt}
  \multicolumn{2}{c|}{Method} & MTG-pair & JoJoGAN-pair & Ours\\ \Xhline{0.6pt}
  \multirow{3}*{Example-1} & LPIPS $\downarrow$ &  0.423 & \underline{0.381} & \textbf{0.353} \\
  ~ & dir-CC $\uparrow$  & \underline{0.195} & 0.180 & \textbf{0.196} \\
  ~ & dir-ID $\uparrow$ & 0.392 & \underline{0.405} & \textbf{0.468} \\ \Xhline{0.6pt}
  \multirow{3}*{Example-2} & LPIPS $\downarrow$ & 0.447 & \underline{0.395} & \textbf{0.379} \\
  ~ & dir-CC $\uparrow$ & \underline{0.174} & 0.155 & \textbf{0.194} \\
  ~ & dir-ID $\uparrow$ & 0.335 & \textbf{0.393} & \underline{0.379} \\ \Xhline{0.6pt}
  \multirow{3}*{Example-3} & LPIPS $\downarrow$ & \underline{0.379} & 0.383 & \textbf{0.342} \\
  ~ & dir-CC $\uparrow$ & 0.159 & \underline{0.173} & \textbf{0.191} \\
  ~ & dir-ID $\uparrow$ & 0.280 & \textbf{0.400} & \underline{0.330} \\ \Xhline{1pt}

\end{tabular} 
\end{center}
% \end{minipage}
\vspace*{-3mm}
\end{table}%
%\vspace{-0.3cm}

==> tables/eval_unpair.tex <==

\begin{table*}[htbp]%
\small 
\caption{
\textbf{Quantitative comparison.} We choose the three styles shown in Fig.~\ref{fig:cmp_unpair} for evaluation, denoted as Example-1, Example-2 and Example-3. Part I shows the comparison with existing one-shot methods trained with only the style reference, whereas Part II lists the comparison with the ``paired'' variants of MTG~\cite{zhu2022mtg} and JoJoGAN~\cite{chong2022jojogan}. Note the best results are \textbf{blod}, and the second-bests are \underline{underlined}. 
} % of methods by three metrics
\label{tab:eval_unpair}
% \begin{minipage}{\columnwidth}
\vspace*{-5mm}
\begin{center}
\begin{tabular}{c|c|ccc|ccc|ccc}

  \Xhline{1pt}
  & \multirow{2}*{Method} & \multicolumn{3}{c|}{Example-1} & \multicolumn{3}{c|}{Example-2} & \multicolumn{3}{c}{Example-3} \\ \cline{3-11}
  & ~ & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} & LPIPS $\downarrow$ & \makecell{dir-CC $\uparrow$} & \makecell{dir-ID $\uparrow$} \\ \Xhline{0.6pt}
  \multirow{5}*{\textbf{\uppercase\expandafter{\romannumeral1}}} & MTG \cite{zhu2022mtg} & \textbf{0.340} & 0.123 & 0.264 & \underline{0.361} & 0.111 & 0.301 &\textbf{0.328} & 0.095 & 0.254 \\
  & JoJoGAN \cite{chong2022jojogan} & 0.357 & 0.149 & 0.290 & 0.385 & \underline{0.138} & 0.378 & 0.355 & 0.097 & \textbf{0.382} \\
  & DiFa \cite{zhang2022towards} & 0.362 & 0.142 & 0.223 & \textbf{0.293} & 0.137 & 0.328 & 0.346 & 0.094 & 0.123 \\
  & OneshotCLIP \cite{guhyun2023oneshotclip} & 0.452 & \underline{0.157} & \underline{0.333} & 0.449 & 0.119 & 0.113 & 0.460 & \underline{0.136} & 0.201 \\ \cline{2-11}
%   MTG-pair & 0.423 & \underline{0.195} & 0.392 & 0.447 & \underline{0.174} & 0.335 & 0.379 & 0.159 & 0.280 \\
%   JoJoGAN-pair & 0.381 & 0.180 & \underline{0.405} & 0.395 & 0.155 & \textbf{0.393} & 0.383 & \underline{0.173} 
% & \textbf{0.400} \\ \cline{1-10}
  & Ours & \underline{0.353} & \textbf{0.196} & \textbf{0.468} & 0.379 & \textbf{0.194} & \textbf{0.379} & \underline{0.342} & \textbf{0.191} & \underline{0.330} \\
  
  \hline\hline

  \multirow{3}*{\uppercase\expandafter{\romannumeral2}} & MTG-pair & 0.423 & \underline{0.195} & 0.392 & 0.447 & \underline{0.174} & 0.335 & \underline{0.379} & 0.159 & 0.280 \\
   & JoJoGAN-pair & \underline{0.381} & 0.180 & \underline{0.405} & \underline{0.395} & 0.155 & \textbf{0.393} & 0.383 & \underline{0.173} 
 & \textbf{0.400} \\ \cline{2-11}
  & Ours & \textbf{0.353} & \textbf{0.196} & \textbf{0.468} & \textbf{0.379} & \textbf{0.194} & \underline{0.379} & \textbf{0.342} & \textbf{0.191} & \underline{0.330} \\
  \Xhline{1pt}
  % \hline
\end{tabular} 
\end{center}
% \end{minipage}
\vspace*{-3mm}
\end{table*}%
%\vspace{-0.3cm}
